Unsupervised Machine Learning for Detecting and Locating Human-Made Objects in 3D Point Cloud

A 3D point cloud is an unstructured, sparse, and irregular dataset, typically collected by airborne LiDAR systems over a geological region. Laser pulses emitted from these systems reflect off objects both on and above the ground, resulting in a dataset containing the longitude, latitude, and elevation of each point, as well as information about the corresponding laser pulse strengths. A widely studied research problem, addressed in many previous works, is ground filtering, which involves partitioning the points into ground and non-ground subsets. This research introduces a novel task: detecting and identifying human-made objects amidst natural tree structures. This task is performed on the subset of non-ground points derived from the ground filtering stage. Marked Point Fields (MPFs) are used as models well-suited to these tasks. The proposed methodology consists of three stages: ground filtering, local information extraction (LIE), and clustering. In the ground filtering stage, a statistical method called One-Sided Regression (OSR) is introduced, addressing the limitations of prior ground filtering methods on uneven terrains. In the LIE stage, unsupervised learning methods are lacking. To mitigate this, a kernel-based method for the Hessian matrix of the MPF is developed. In the clustering stage, the Gaussian Mixture Model (GMM) is applied to the results of the LIE stage to partition the non-ground points into trees and human-made objects. The underlying assumption is that LiDAR points from trees exhibit a three-dimensional distribution, while those from human-made objects follow a two-dimensional distribution. The Hessian matrix of the MPF effectively captures this distinction. Experimental results demonstrate that the proposed ground filtering method outperforms previous techniques, and the LIE method successfully distinguishes between points representing trees and human-made objects.

==> paper/discussion.tex <==
\section{Extensions of SBR}
SBR is not limited to linear regression and one categorical variable. It can also be applied to other regression problems and datasets with multiple categorical variables. Besides, as it can verify the hypothesis test in \eqref{eq:h0} and calculate $F$-statistics, it can also be used to calculate multiple models simultaneously.

\subsection{Other Regression Problems}
SBR can also be applied to other regression problems, such as Box-Cox linear regression ~\cite{box1964analysis}. Box-Cox linear regression is linear regression with response variables transformed by Box-Cox parameter $c$, as is shown in \eqref{eq:bcreg_pp}.
\begin{align} \label{eq:bcreg_pp}
    \mathbf{y}^{(c)}=
    \begin{cases}
        (\mathbf{y}^c-1)/c \text{ if $c \neq 0$ } \\
        \log \mathbf{y} \text{ if $c=0$ }
    \end{cases}
\end{align}

Additionally to the calculation of the sparse block matrix of $\mathcal{S}$, $s_{logy}=(c-1)\sum_{i=1}^{I}\sum_{j=1}^{n_i}y_{ij}$ is also needed to calculate the profile loglikelihood of Box-Cox linear regression. $c$ is the Box-Cox parameter.

A big data version of SBR for Box-Cox linear regression is shown in \algorithmref{alg:sbr_bc_bigdata}.

\begin{algorithm}[tb]
\caption{SBR for Box-Cox Transformation}
\label{alg:sbr_bc_bigdata}
\begin{flushleft}
\textbf{Input}: $R$ RDDs partitioned from the entire dataset, Box-Cox parameter $c$ \\
% \textbf{Parameter}: Optional list of parameters\\
\textbf{Output}: $\hat{\bm{\gamma}}_1$, $\hat{\bm{\gamma}}_2$, $\dots$, $\hat{\bm{\gamma}}_I$, $\hat{\bm{\delta}}^2$, $\hat{\sigma}^2$ and $\hat{\rm{V}}(\hat{\bm{\delta}})$
\end{flushleft}
\begin{algorithmic}[1] %[1] enables line numbers
    \Procedure{Mapper}{$r$th RDD of the dataset}
        \State $s_{r,yy}=0, s_{r,logy}=0,\mathbf{S}_{r,wy}=\mathbf{0}, \mathbf{S}_{r,zy}=\mathbf{0}$
        \State $\mathbf{S}_{r,ww}=\mathbf{0}, \mathbf{S}_{r,wz}=\mathbf{0}, \mathbf{S}_{r,zz}=\mathbf{0}$
        \For{$i \gets 0$ to $I-1$}
            \State $\mathbf{S}_{r,wy}[i]=\mathbf{0}, \mathbf{S}_{r,zy}[i]=\mathbf{0}, \mathbf{S}_{r,ww}[i]=\mathbf{0}$ 
            \State $\mathbf{S}_{r,wz}[i]=\mathbf{0}, \mathbf{S}_{r,zz}[i]=\mathbf{0}$
        \EndFor
        \For{$j$th elements $\gets$ RDD}
            \State $i \gets $ level of $j$th observation
            \State $s_{j,yy}=(y_{j}^{(c)})^2, s_{j,logy}=\log y$ \State $\bm{s}_{j,wy}=\bm{w}_{j}y_{j}^{(c)}, \bm{s}_{j,zy}=\bm{z}_{j}y_{j}^{(c)}$
            \State $\mathbf{S}_{j,ww}=\bm{w}_{j}^\top \bm{w}_{j}, \mathbf{S}_{j,wz}=\bm{w}_{j}\bm{z}_{j}^\top$
            \State $\mathbf{S}_{j,zz}=\bm{z}_{j}\bm{z}_{j}^\top$
            \State $s_{r,yy}\pluseq s_{j,yy},s_{r,logy}\pluseq s_{j,logy}$
            \State $\mathbf{S}_{wy}[i] \pluseq \mathbf{s}_{j,wy}, \mathbf{S}_{r,zy}[i] \pluseq \bm{s}_{j,zy}$
            \State $\mathbf{S}_{r,ww}[i] \pluseq \mathbf{S}_{j,ww},\mathbf{S}_{r,wz}[i] \pluseq \mathbf{S}_{j,wz}$
            \State $\mathbf{S}_{r,zz}[i] \pluseq \mathbf{S}_{j,zz}$
        \EndFor
        \State \textbf{return} $r$th RDD
    \EndProcedure
    \Procedure{Reducer}{$c$,$R$ RDDs from Mapper}
        \State $s_{yy}=0, s_{logy}=0, \mathbf{S}_{wy}=\mathbf{0}, \mathbf{S}_{zy}=\mathbf{0}$
        \State $\mathbf{S}_{ww}=\mathbf{0}, \mathbf{S}_{wz}=\mathbf{0}, \mathbf{S}_{zz}=\mathbf{0}$
        \For{$r \gets 0$ to $R-1$}
            \State $s_{yy}\pluseq s_{r,yy}$
            \State $s_{logy}\pluseq (c-1)s_{r,logy}$
            \For{$r \gets 0$ to $R-1$}
                \State $\mathbf{S}_{wy}[i]\pluseq \mathbf{S}_{r,wy}[i], \mathbf{S}_{zy}[i]\pluseq\mathbf{S}_{r,zy}[i]$
                \State $\mathbf{S}_{ww}[i]\pluseq\mathbf{S}_{r,ww}[i],\mathbf{S}_{wz}[i]\pluseq\mathbf{S}_{r,wz}[i]$ 
                \State $\mathbf{S}_{zz}[i]\pluseq\mathbf{S}_{r,zz}[i]$
            \EndFor
        \EndFor
    \EndProcedure
    \Procedure{Main}{$c$}
        \State Collect $\mathcal{S}$ from $Mapper$ and $Reducer$
        \State Compute $\hat{\bm{\gamma}}_1$,\dots, $\hat{\bm{\gamma}}_I$, $\hat{\sigma}^2$, $\hat{\bm{\delta}}$, $\hat{\sigma}^2$ and $\hat{\rm{V}}(\hat{\bm{\delta}})$
    \EndProcedure
\end{algorithmic}
\end{algorithm}

\subsection{Multiple Categorical Variables}
Assume $A$ and $B$ be two categorical variables with $I$ and $J$ levels respectively. The dataset can be expressed as:
\begin{align} \label{eq:two_level_D}
\begin{split}
    \mathcal{D}= & \{(y_{ijk},\bm{x}^\top_{ijk},A_i,B_j): \\
    & i=1,\dots,I,j=1,\dots,J,k=1,\dots,n_{ij}\}
\end{split}
\end{align}
where $\bm{x}_{ijk}=(1,x_{ijk1},x_{ijk2},\dots,x_{ijk(q-1)}^\top)$ represents the $(i,j,k)$th observation.

Based on \eqref{eq:two_level_D}, we could treat the two categorical variables $A$ and $B$ as one categorical variable $L$ with $IJ$ levels. 
\begin{align} \label{eq:two_level_one}
\begin{split}
    \mathcal{D}= & \{(y_{ik},\bm{x}^\top_{ik},L_i): \\
    & i=1,\dots,IJ,k=1,\dots,n_i\}
\end{split}
\end{align}
where $\bm{x}_{ijk}=(1,x_{ijk1},x_{ijk2},\dots,x_{ijk(q-1)}^\top)$ represents the $(i,j,k)$th observation. Based on the definiton of the spase block matrix from \eqref{eq:sparse_block_matrix}, we could find a matrix $\mathcal{S}$ to derive the model coefficients.

Likewise, SBR is applicable for datasets with three or more categorical variables. 
